Reparo: Loss-Resilient Generative Codec for Video Conferencing

Packet loss during video conferencing often results in poor quality and video freezing. Retransmitting lost packets is often impractical due to the need for real-time playback, and using Forward Error Correction (FEC) for packet recovery is challenging due to the unpredictable and bursty nature of Internet losses. Excessive redundancy leads to inefficiency and wasted bandwidth, while insufficient redundancy results in undecodable frames, causing video freezes and quality degradation in subsequent frames. We introduce Reparo -- a loss-resilient video conferencing framework based on generative deep learning models to address these issues. Our approach generates missing information when a frame or part of a frame is lost. This generation is conditioned on the data received thus far, considering the model's understanding of how people and objects appear and interact within the visual realm. Experimental results, using publicly available video conferencing datasets, demonstrate that Reparo outperforms state-of-the-art FEC-based video conferencing solutions in terms of both video quality (measured through PSNR, SSIM, and LPIPS) and the occurrence of video freezes.

==> Makefile <==
.PHONY: all clean dist print

P = main

default : $P.pdf

$P.dvi	: $(wildcard *.tex source/*.tex *.bib figures/*.eps)
	latex  $P < /dev/null || $(RM) $@
	bibtex $P < /dev/null || $(RM) $@
	latex  $P < /dev/null || $(RM) $@
	latex  $P < /dev/null || $(RM) $@

onerun  : $(wildcard *.tex source/*.tex *.bib figures/*)
	bibtex $P
	pdflatex --shell-escape $P

$P.pdf  : $(wildcard *.tex source/*.tex *.bib figures/*)
	pdflatex --shell-escape $P
	bibtex $P
	pdflatex --shell-escape $P
	pdflatex --shell-escape $P
	
embedded:
	gs -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress \
	    -dEmbedAllFonts=true \
	    -sOutputFile=$P_embedded.pdf \
	    -f $P.pdf

$P.ps	: $P.dvi
	dvips -tletter -Ppdf $P.dvi -o $P.ps
	ps2pdf -dPDFSETTINGS=/prepress -dEmbedAllFonts=true $P.ps

$P.ps.gz: $P.ps
	$(RM) $P.ps.gz
	gzip -9 < $P.ps > $P.ps.gz

print:	$P.ps

dist:	$P.ps.gz

clean:
	$(RM) $P.pdf $P.log $P.aux $P.bbl $P.blg $P.out $P.dvi $P.ps $P.ps.gz texput.log $P_embedded.pdf


==> source/abstract-0.tex <==
\begin{abstract}

% Packet loss degrades the quality of experience (QoE) of videoconferencing. This is because the commonly used real-time video codecs such as VP9 are not resilient to losses. As a result, once a packet is lost, the decoder failed to decode the corresponding frame. Moreover, those codecs typically have a high temporal dependency. As a result, one un-decodable frame could cause multiple subsequent frames to be un-decodable as well, leading to video freezes which largely degrades QoE of videoconferencing.

% The current approach to recover lost packets where retransmission takes too long is forward error correction (FEC), where the sender needs to send redundant data to help the receiver recover lost packets. However, such schemes just reduce the amount of un-decodable frames. Once a lost data packet cannot be recovered, due to the limitations of traditional video codec, it will still cause the video to freeze. In this paper, we propose \name, a neural-based loss-resilient codec that overcomes the aforementioned limitations of traditional video codecs.
% It consists of three parts: an encoder, a decoder, and a loss reconstruction module. The encoder and decoder are both temporal independent, and the loss reconstruction module is used to reconstruct lost packets. Therefore, one un-decodable frame will not affect the subsequent frames. Moreover, unlike FEC which requires large bandwidth overhead, our loss reconstruction module exploits both spatial and temporal redundancy of the encoded video and introduces no bandwidth overhead.
% We evaluate \name~on standard benchmarks in the videoconferencing literature \cite{xxx} and evaluate end-to-end QoE metrics over an emulated network. \name~improves the average PSNR of received video by xxx dB and 90 percentile PSNR by xxx dB, and reduces the cumulative duration of freezes to almost 0.

Video conferencing quality of experience (QoE) is often degraded by packet loss, as commonly used real-time video codecs like VP9 are highly temporally dependent and not resilient to packet or frame losses. This results in frames that cannot be decoded and subsequent freezes, which greatly affect the QoE. Although forward error correction (FEC) schemes help reduce the number of un-decodable frames, it cannot prevent the video from freezing once a packet is lost.
To address this problem, we propose \name, a neural loss-resilient codec consisting of an encoder, decoder, and loss reconstruction module. Unlike traditional video codecs, both the encoder and decoder of \name~are temporally independent, while the loss reconstruction module reconstructs lost packets by exploiting spatial and temporal redundancy without introducing bandwidth overhead. As a result, most lost packets can be recovered, and an un-decodable frame will not affect any subsequent frames.
We evaluate \name~on a standard video conferencing benchmark and measure end-to-end QoE metrics over an emulated network. \name~improves the average and 90th percentile PSNR of received video by a large margin across different loss levels, and nearly eliminates freezes.

\end{abstract}


==> source/intro-0.tex <==
\section{Introduction}

Packet loss is a major issue in internet-based video conferencing. Even losing a single packet can prevent the rendering of a video frame, and can also hinder the rendering of future frames due to inter-frame dependencies which are common in modern video codecs. There are two broad solutions to this problem: retransmissions and forward error correction (FEC). However, since video conferencing applications must recover lost packets within a strict latency to meet the real-time playback requirement, retransmission is only suitable for scenarios with short round trip times. In all other cases, video conferencing applications rely on FEC to recover lost packets within an acceptable latency.

FEC relies on sending redundant packets, known as the "parity" packets, to recover the lost "data" packets. However, current FEC schemes have two major limitations. First, if one frame is un-decodable due to a bursty loss \cite{xxx}, such a frame could still result in many subsequent frames being non-rendered due to inter-frame dependencies. This typically causes the video conferencing to freeze, which largely affects the QoE. Second, one frame is decodable only if the data packets for that frame can all be recovered. As a result, all FEC schemes need large bandwidth overheads to transmit the parity packets to recover lost data packets.

Recently, researchers found that there is extensive spatial redundancy in natural images. For instance, in recent visual self-supervised learning based on reconstructive learning, researchers found that a neural network can learn to reconstruct an image whose 75\% of pixels are masked. This shows that a small subset of the pixels of an image could contain almost the same amount of information as the original image. Another line of work, such as VQVAE and VQGAN, focuses on compressing images into discrete visual token maps that could reconstruct the original images. They found that natural images can be compressed to visual token maps with a much smaller resolution using a vector-quantized auto-encoder. Moreover, MAGE \cite{xxx} found that such highly-compressed token maps could be further masked, and the remaining tokens can still reconstruct the original image.

Inspired by this, we propose \namereparo, a novel loss recovery scheme that is completely different from previous schemes based on FEC. We observe that the aforementioned two limitations of current FEC schemes are actually caused by the temporal-dependent video codec that all FEC schemes build on, such as VP9. Therefore, instead of using a temporal-dependent video codec that is not resilient to losses, we propose to use a temporal-independent neural codec to first encode each frame into visual token maps -- i.e., we encode and decode each frame independently. This solves the first problem that one un-decodable frame could cause several subsequent frames to be non-rendered, even if they receive all their data packets. Moreover, as shown in \Sec{results}, such a codec will not introduce a large bandwidth overhead because video conferencing is a specific domain containing mostly human face images. Therefore, the neural codec can be focused on such a domain and achieve high PSNR with a large compression ratio.

With the video transferred into visual token maps, we further use a spatiotemporal reconstruction module on the receiver side to reconstruct any lost tokens. Such a reconstruction module exploits both the spatial and temporal redundancy of the video. For example, a visual token at the same position in two consecutive frames could be very similar. As a result, if one of the two tokens is lost, the reconstruction module can easily reconstruct it. Similarly, a visual token also could be inferred by its surrounding tokens. Such a design solves the second problem -- even if only a subset of tokens from one frame is received, the reconstruction module can still reconstruct the lost tokens and decode the whole frame.

Besides resolving the two aforementioned limitations of traditional FEC schemes, \namereparo~also brings multiple additional advantages. First, traditional video codecs require a high bitrate whenever a keyframe is forced either by the codec or by the receiver to recover from un-decodable frames. On the other hand, \namereparo~operates on a constant bitrate -- every frame is encoded into a token map with a fixed size. Second, it can be easily adapted to different target bitrates. Second, it is hard to adjust traditional video codecs to meet an exact target bitrate. The actual bitrate will always fluctuate during the transmission. However, \namereparo~can easily adapt to different target bitrates by simply randomly dropping during packetization \Sec{packetization}. Therefore, it can always transmit at the target bitrate constantly.

Another advantage of \namereparo~is that it only needs one-way communication. In traditional FEC schemes, the receiver will send an ACK for every decodable frame to the transmitter. This causes two problems: if the ACK is lost, the transmitter will force a new keyframe which introduces large bandwidth overhead. And to recover from an un-decodable frame, the sender will wait for the ACK for that frame to time out. This could cause even longer freezes when the round-trip time is long. However, in \namereparo, the receiver does not need to communicate with the transmitter about un-decodable frames -- it will always use the received tokens to reconstruct the lost ones, and even if one frame cannot be recovered, it will simply wait for the next frame and render it.

We evaluate \namereparo~on a dataset consisting of publicly available video conferencing videos on YouTube, using the officially released Tambur evaluation platform \cite{xxx} under different bitrate constraints and loss levels. We compare \namereparo's performance with VP9+Tambur, which is one of the state-of-the-art FEC schemes based on streaming code, and evaluate the PSNR of the displayed video. The results show that \namereparo~consistently outperforms VP9+Tambur at different loss levels. It achieves a similar PSNR as VP9+Tambur when the loss is mild, while significantly improving over VP9+Tambur when the loss is heavy. Specifically, \namereparo~achieves 34.1 dB, 34.0 dB, and 33.9 dB 90 percentile PSNR under low, medium, and high loss levels, which outperforms VP9+Tambur by 3.1 dB, 9.8 dB, and 17.9 dB, respectively. It further mostly eliminates video freezes, with the percentage of non-rendered frames to be 0.2\%, 0.8\%, and 2.0\% under low, medium, and high loss levels.

We summarize our contributions as follows:

\begin{Itemize}
    \item We identify two major limitations of current FEC-based loss recovery schemes to reside in the design of traditional video codec, and highlight a completely different potential direction for loss-resilient video conferencing.
    \item We introduce \namereparo, the first loss-resilient neural video codec for video conferencing. \namereparo~proposes a new structure of neural video codec, where the encoder and decoder are temporally independent, and a loss reconstruction module is introduced to exploit spatial and temporal redundancy. Such a design allows the system to quickly recover from a non-rendered frame due to packet losses, which mostly eliminates video freezes.
    \item We implement \namereparo~and integrate it with a benchmark video conferencing platform for evaluating FEC schemes. We further evaluate \namereparo~on a benchmark dataset and show significant improvements over key metrics pertaining to end-to-end QoE, such as PSNR and frequency of non-rendered frames.
\end{Itemize}

==> source/intro-1.tex <==
\section{Introduction}

Traditional video codecs create a strong dependency between encoded frames. For exampe, P-frames depend on previous frames, and  to decode them, the receiver must first decode the frames on which it depends. If those frames cannot be decoded due to lost packets, the receiver stalls and cannot proceed, causing the video to freeze. The only way to make progress is to either receive the missing data and decode the needed frames, or to give up and request a new key frame (called I-frame). The I-frame effectively resets the state of the decoder, and subsequent frames can then be encoded with respect to this new state. However, since I-frames must be compressed independently of other frames, they are much larger than P-frames, and so the I-frame is usually sent at a lower quality to mitigate the spike in bitrate. This not only affects the I-frame's quality but also the quality of subsequent frames. The overall result is that packet loss episodes can cause a jarring user experience where the video freezes followed by a period of poor quality until the codec recovers. 

There are two broad techniques to combat this problem in existing systems: retransmission and forward error correction (FEC). Since real-time applications such as video conferencing must recover lost packets within a limited latency to meet the real-time playback requirement, retransmission is only suitable for scenarios with short round trip times. In all other cases, such applications rely on FEC to recover lost packets within an acceptable latency. FEC schemes send redundant packets, known as ``parity'' packets, to recover the lost data using traditional block codes \cite{reed1960polynomial, mackay2005fountain} or latency-optimized streaming codes~\cite{tambur}. However, all FEC approaches face a challenge in choosing how much redundancy to add since losses in the Internet are bursty and unpredictable. Too much redundancy leads to inefficiency and wasted bandwidth, and too little redundancy leads to undecodable frames, causing video freezes and quality issues on subsequent frames. 

%It is evident that the strict dependencies between frames makes existing systems highly vulnerable to packet loss. Instead, if we could decode each frame based on whatever data has been received up to that point, we could be much more resilient to packet loss. Such a system would never stall due to missing packets from a frame; it would simply proceed an

In this paper, we take a different approach to loss recovery in video conferencing. We neither send redundant packets nor ask for retransmission. When a loss occurs, the receiver simply tries its best to ``generate'' the missing information. To do so, we build on recent advances in generative deep learning models. Generative models can reconstruct realistic images from a small amount to zero data. For example, they can reconstruct an image even if 75\% of the pixels are missing \cite{MAE, li2022mage}. Unlike traditional video codecs, which use only the received data to reconstruct the source information, generative models operate like humans; they use the wealth of knowledge on how people look, dress, and move to generate missing information. For example, seeing a person's eye, they can generate the other eye, and with a glimpse of one's arm, they can generate the whole torso. Our insight is that such generative models are a natural fit for loss-resilient video conferencing. In particular, since generative models can predict missing information from their knowledge of the visual world, they can accurately generate the lost content. 

%In particular, since generative models can predict missing information from their knowledge of the visual world, they can compress videos in a domain such as video conferencing extremely well without relying on temporal locality between frames. We show that this enables a codec design that sidesteps the pitfalls of inter-dependent frames entirely.

%\tianhong{Geneartive models do not allow us to encoder frames independently (that's done by the codec), but allow us to reconstruct lost data.}

We introduce \namereparo, a loss-resilient generative codec for video conferencing.  The design of \namereparo\ involves two steps. In the first step, we learn how to represent the world of video conferencing frames using a small dictionary of visual tokens, where each token refers to a patch in a frame. The objective of this step is to capture how visual objects look and relate to each other through a small number of abstract tokens and their relationships. \namereparo\ then operates on tokens. The transmitter uses a neural network to encode each frame into its set of tokens, which it packetizes and transmits. Some of these packets may get lost in the network. The \namereparo\ receiver has a neural network that can regenerate the missing tokens from those that it receives and its knowledge of how tokens relate to each other in the visual world. Finally, the reconstructed tokens are decoded to produce the original frame. \Fig{overview} illustrates the components of \namereparo.

Beyond eliminating the need for transmitting redundant packets, \namereparo\ offers three additional advantages. First, it can compress the video efficiently without creating dependencies between transmitted frames. This is because although \namereparo does not leverage temporal relationships across frames for compression, it captures the prevalent visual features and dependencies between objects and shapes in video conferencing frames within its codebook, which is learned ahead of time and is known to both the transmitter and receiver. During transmission, \namereparo\ need only send token indices as opposed to the actual tokens and the underlying dependencies. 

Second, traditional video codecs have a highly variable bit rate since keyframes are much larger than other frames. As a result, it is difficult for traditional video codecs to meet an exact target bitrate, and the actual bitrate will always fluctuate during transmission. In contrast, in \namereparo, all frames are equal, and hence \namereparo\ operates at a constant bitrate and can easily adapt to any target bitrate.
%\vls{we should commit to either ``bit rate'' or ``bitrate''; the paper uses both atm}. \ma{I think bitrate is correct. Let's use that}

Third, \namereparo\ requires only one-way communication. In past video-conferencing FEC schemes~\cite{tambur}, the receiver sends an ACK for every decodable frame. The sender waits for the ACK to retransmit, which could cause even longer freezes when the round-trip time is long. In contrast, in \namereparo, the receiver does not need to communicate with the transmitter about undecodable frames; it will always use the received tokens to reconstruct the lost ones. Even if one frame cannot be recovered, it will simply wait and render the next frame.

\red{We compare \namereparo~with FEC schemes integrated with WebRTC \cite{webrtc} (ULPFEC and flexFEC), as well as Tambur, a state-of-the-art streaming-code-based FEC approach. We evaluate them on a large and diverse corpus of publicly available video conferencing style videos (more than 5 hours of videos from 84 people). The results show the following}:
\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
\item \namereparo\ consistently improves the visual quality of displayed videos over baselines for all loss levels. 
%It achieved similar PSNR as VP9+Tambur under mild loss conditions and significantly outperformed VP9+Tambur under heavy loss conditions. 
Specifically, \namereparo\ achieves 34.1 dB, 34.0 dB, and 33.9 dB 10\textsuperscript{th} percentile PSNR under low, medium, and high loss levels, respectively, outperforming state-of-the-art VP9+Tambur by 3.1 dB, 9.8 dB, and 17.9 dB. %This difference in PSNR is typically noticeable, as a 1 dB difference is perceivable.

%\item \namereparo\ nearly eliminates all video freezes, with the percentage of non-rendered frames being only 0.2\%, 0.8\%, and 2.0\% under low, medium, and high loss levels, respectively when VP9+Tambur experiences significantly more non-rendered frames for all loss levels.
\item \namereparo\ nearly eliminates all video freezes, failing to render only 0.2\%, 0.8\%, and 2.0\% of frames under low, medium, and high loss levels, respectively, when Tambur fails to render significantly more frames for all loss levels (up to 29.2\% of frames at high loss).

\item \namereparo\ transmits at a constant bitrate and adapts to a range of target bitrates smoothly. %This provides an advantage over VP9+Tambur in scenarios where there is a rate-limited link in the network. 
In rate-limited environments, \namereparo\ utilizes the full capacity of the link, while VP9+Tambur needs to keep the average bitrate low to avoid packet losses due to the high variability of the VP9 encoder's bitrate.

\end{enumerate}

Overall, \namereparo achieves superior loss-resilience and quality stability compared to existing approaches. One limitation, however, is that \namereparo is more computationally intensive than traditional methods. It requires high-end GPUs to operate in real time which are typically only available on high-end laptops. A wealth of techniques have been proposed in recent years to improve the computational efficiency of neural networks. We leave an exploration of such techniques to make \namereparo accessible to a wider range of devices for future work. Nevertheless, \namereparo presents a promising approach to loss-resilient video conferencing and we hope it opens up further research in this area.

Can be run on GPUs equivalent to a laptop


\if 0
Traditional video codecs have a strong time dependence, where frames are encoded with respect to earlier data (e.g., P frames are coded with respect to I frames). This dependence makes them highly vulnerable to packet loss, where a loss not only affects the current frame but could also impact later data that was coded with respect to the lost packets. There are two broad solutions to this problem: retransmissions and forward error correction (FEC). However, since video conferencing must recover lost packets within limited latency to meet the real-time playback requirement, retransmission is only suitable for scenarios with short round trip times. In all other cases, video conferencing applications rely on FEC to recover lost packets within an acceptable latency. FEC schemes send redundant packets, known as ``parity'' packets, to recover the lost data. However, the transmitter cannot choose an optimal amount of redundancy since losses in the Internet are bursty and unpredictable. Too much redundancy leads to inefficiency and low quality, and too little redundancy leads to unrendered frames and hence video freezes and corruption.

In this paper, we take a different approach to loss recovery in video conferencing. We neither send redundant packets nor ask for retransmission. When a loss occurs, the receiver simply tries its best to recover the missing information. To do so, we build on recent advances in generative deep learning models. Generative models can reconstruct realistic images from a small amount to zero data. For example, they can reconstruct an image even if 75\% of the pixels are missing \cite{MAE, li2022mage}. Unlike traditional video codecs, which use only the received data to reconstruct the source information, generative models operate like humans; they use the wealth of knowledge on how people look, dress, and move to generate missing information. For example, seeing a person's eye, they can generate the other eye, and with a glimpse of one's arm, they can generate the whole torso. Our insight is that such generative models are a natural fit for loss-resilient video conferencing.

We introduce \namereparo, a loss-resilient generative codec for video conferencing. %video streaming architecture.  
The design of \namereparo\ involves two steps. In the first step, we learn how to represent the whole world of video conferencing frames using a small dictionary of visual tokens, where each token refers to a patch in a frame. The objective of this step is to capture how visual objects look and relate to each other through a small number of abstract tokens and their relationships. \namereparo\ then operates on tokens. The transmitter uses a neural network to encode each frame into its set of tokens, which it packetizes and transmits. Some of these packets may get lost in the network. The \namereparo\ receiver has a neural network that can regenerate the missing tokens from those that it receives and its knowledge of how tokens relate to each other in the visual world. Finally, the reconstructed tokens are decoded to the original frame. \Fig{overview} illustrates the components of \namereparo.

Beyond eliminating the need for transmitting redundant packets, \namereparo\ offers two additional advantages. First, traditional video codecs have a highly variable bit rate since keyframes are much larger than other frames. As a result, it is difficult for traditional video codecs to meet an exact target bitrate, and the actual bitrate will always fluctuate during transmission. In contrast, in \namereparo, all frames are equal, and hence \namereparo\ operates at a constant bit rate and can easily adapt to any target bit rate.

Second, \namereparo\ requires only one-way communication. In past video-conferencing FEC schemes \cite{tambur}, the receiver sends an ACK for every decodable frame. The sender waits for the ACK to retransmit, which could cause even longer freezes when the round-trip time is long. In contrast, in \namereparo, the receiver does not need to communicate with the transmitter about undecodable frames -- it will always use the received tokens to reconstruct the lost ones, and even if one frame cannot be recovered, it will simply wait for the next frame and render it.

We evaluate \namereparo\ on a dataset consisting of publicly available video conferencing videos on YouTube. We compare \namereparo's performance with VP9+Tambur, a state-of-the-art loss-resilient video conferencing platform based on streaming FEC. The results show that \namereparo\ consistently outperforms VP9+Tambur for all loss levels. It achieves a similar PSNR as VP9+Tambur when the loss is mild, while significantly improving over VP9+Tambur when the loss is heavy. Specifically, \namereparo\ achieves 34.1 dB, 34.0 dB, and 33.9 dB 10 percentile PSNR under low, medium, and high loss levels, respectively, which outperforms VP9+Tambur by 3.1 dB, 9.8 dB, and 17.9 dB. It further mostly eliminates video freezes, with the percentage of non-rendered frames being 0.2\%, 0.8\%, and 2.0\% under low, medium, and high loss levels.
\fi 

==> source/method-0.tex <==
\begin{figure}[t]
\begin{center}

\includegraphics[width=1.0\linewidth]{figures/overview}
\end{center}
\caption{Overview of \namereparo. A discrete encoder-decoder pair convert between RGB image and quantized image tokens, while we introduce new modules to affect the packetization, bitrate, and loss recovery in the quantized token space to improve loss-resilience.}\label{fig:overview}
\end{figure}

\section{\namereparo Design}
\label{sec:design}

\subsection{Overview}
\label{sec:design overview}
\namereparo is a neural loss-resilient video codec specifically designed for video conferencing. As shown in \Fig{overview}, \namereparo~consists of five parts: (1) a \emph{discrete encoder} based on the VQGAN~\cite{esser2021taming} architecture that encodes the RGB video frame into a set of discrete tokens (that are mapped to continuous features via a \emph{codebook}, (2) a \emph{deterministic packetizer} that organizes the tokens into a sequence of packets in a way that minimizes the impact of lost packets once transmitted across the network,  (3) a \emph{bitrate controller} that adaptively drops some fraction of the discrete packetized tokens to achieve a target bitrate, (4) a \emph{loss recovery module} that is responsible for reconstructing the remaining tokens in their appropriate positions based on what was actually received by the receiver within its frame deadline, and (5) a \emph{discrete decoder} that maps the reconstructed tokens back to features using the codebook, and decodes the features into RGB frame. We call the encoder-decoder combination in \namereparo~its neural codec, while the rest of the components help it with loss recovery atop the codec. We describe each module in detail below.
%The transmitter uses a neural-based video encoder to compress each frame of the raw video into a highly-compressed token map consisting of visual tokens. 2. The transmitter wraps the token map of each frame into several packets to be transmitted over the network. 3. Once the receiver hits the deadline for displaying a frame, it regards all unreceived packets as lost and decode the token map from received packets. It then uses the received tokens to recover those lost tokens through the loss reconstruction module. 4. The receiver uses a neural-based video decoder to decode the reconstructed token map to RGB frame. Below, we will describe our token-based neural codec, self-adaptive packetization strategy, and spatiotemporal loss reconstruction module in detail.

%-- Discrete Encoder
%-- Bitrate Control Module
%-- Deterministic Packetization
%-- Loss Recovery Module
%-- Discrete Decoder


\subsection{\namereparo Components}
\label{sec:components}
\subsubsection{Discrete Encoder}
\label{sec:discrete encoder}
\begin{figure}[t]
\begin{center}

\includegraphics[width=1.0\linewidth]{figures/vqgan}

\end{center}
    \caption{Token-based neural codec. The transmitter first uses the encoder to convert video frames into features. It then uses a codebook to quantize the features into tokens by finding the nearest neighbor of each feature in the codebook. The receiver first maps the received and reconstructed tokens to back-to-image features using the codebook. It then uses a decoder to reconstruct the video frame.}
    \label{fig:vqgan}
\end{figure}

\Fig{vqgan} shows the structure of a typical discrete encoder such as VQGAN. The video frame is first encoded into a set of discrete tokens (or image constituents) each of which map to a continuous set of features \ma{I found this sentence confusing.  It would help to refer to the fig more directly. For example, I think you mean to say that the video frame is first divided into a set of $w\times h$ patches each of which map to a continuous $C-$dimensional feature vector. Reserve the word `discrete token' to refer to the learned codewords. And if the term `set of features' just means a C-dimensional feature vector, I would use feature vector rather than set of features. Also, the tokens don't map to continuous features; the continuous features get mapped to the nearest token. I think you want to say something like: The continuous feature vectors are quantized with the help of a learned codebook $Z$ as described below.}. This mapping is stored in a learned \emph{codebook} with each code or token identifier mapping to a specific set of continuous features. The key idea is that images tend to exhibit a lot of redundancy, ensuring that a small set of known features stored in the codebook can be used to construct all details across any image. Since the codebook is learned on specific data with known characteristics, such a codebook can also be finetuned to focus on those features common to a setting, such as facial features for video conferencing. Such approaches have gained popularity in recent days due to their representational power and ease of training~\cite{esser2021taming, yu2021vector, chang2022maskgit, li2022mage}.
%We use a token-based neural codec to encode the input video frames into discrete tokens, which is widely used in the computer vision literature 
 % Such codec consists of the following three parts:

As seen in \Fig{vqgan}, first a convolutional neural network (CNN) encoder $E$ encodes the raw images into low-dimensional features $z \in \mathbb{R}^{C\times h \times w}$, where $C$ is the number of channels in the feature space while $h$ and $w$ denote the height and width respectively. The CNN encoder uses several residual blocks \cite{resnet} to process the video frame, and each block consists of several residual layers. At the end of each block, the feature map is down-sampled by 2 using average pooling. As a result, the encoded features $z$ are of a much lower spatial resolution (16$\times$ or 32$\times$) than the original video frame.

Once the video frame is encoded into a lower-dimensional $z$ vector, a quantizer based on a codebook $Z$ quantizes the features into $\hat{z}$. The codebook $Z$ represents a standard set of image constituents or features to be used to synthesize any high-quality image in a specific domain. Since the mapping is fixed, $\hat{z}$ can be represented by a set of discrete \emph{token indices}, which provides huge compression gains relative to transmitting the features themselves. Every continuous feature in $z$ is mapped to its closest (discrete) neighbor in the codebook $Z$ to generate $\hat{z}$. Each learned codebook $Z$ consists of $N$ tokens, where each token is a feature of $C$ channels. For every pixel $z_{ij}$ in the encoded feature map $z$, we find the token $z_k$ in $Z$ that minimizes the $l_2$ distance between $z_{ij}$ and the selected code. We then use $z_k$ to replace $z_{ij}$ and generate the $h\times w$ token map $\hat{z}$, the quantized version of $z$. The codebook $Z$ itself is learnable and can be optimized for specific settings or image distributions to produce even smaller tokens and greater compression. \ma{This paragraph is good. No need to have the details in the first paragraph.} %Third, a CNN decoder $G$ reconstructs the original video frame based on the quantized features $z_q$. Similar to the CNN encoder, the CNN decoder also consists of several residual blocks. At the end of each block, the feature map is up-sampled by 2 using bicubic interpolation. The CNN decoder has the same amount of residual blocks as the encoder, so it will generate a reconstructed frame with the same shape as the input frame.

% \NewPara{Codebook Generation.} \vls{We have skipped details of how this codebook is actually trained and transmitted for the average video-conferencing call, we need to add that in here. This could posssibly go into a ``Preprocessing'' subsection in 3.3 also}


\subsubsection{Deterministic Packetizer}
\label{sec:packetization}
\begin{figure}[t]
\begin{center}

\includegraphics[width=1.0\linewidth]{figures/packetization}

\end{center}
\caption{The transmitter first uses a deterministic packetizer to wrap image tokens into packets. Then a bitrate controller drops some tokens in each packet to adapt to the target bitrate. The receiver first decodes which tokens are dropped by the bitrate controller. It then depacketizes the received packets to form an image token map with the lost tokens identified.}\label{fig:packetization}
\end{figure}

After encoding the original image into discrete tokens, \namereparo wraps them into several packets to prepare them for transmission. The packetization strategy tries to minimize the redundancy within each packet and maximize the redundancy among different packets. The reason for this is that when a packet is lost, all tokens within the packet are lost. Hence, redundancy within a packet is not as useful. However, redundancy across packets ensures that tokens from a lost packet can be reconstructed from tokens that were successfully received in other packets. Our strategy of wrapping tokens into packets is shown in the first step of \Fig{packetization} in the transmitter for an example with 4$\times$4 tokens that are split into $4$ packets. The packet index of the token at position $(i, j)$ is $2\cdot(i \mod 2) + j \mod 2$. The tokens in one packet are ordered first by its row index, then by its column index in an ascending way. This is just one of many ways to wrap the tokens in a deterministic manner into packets without locality; there are many other ways to achieve the same goal. The key is to ensure that tokens from adjacent squares in the image (which tend to be similar) are spread across multiple packets to enable more resilience to packet loss. The strategy also needs to be deterministic so that the receiver can place the received tokens in the appropriate position before performing loss reconstruction for the missing tokens. Each packet has a header containing its frame index and packet index so that the receiver to identify which frame the tokens belong to, and how many packets that particular frame owns.

%\vls{I don't think the exact mapping of packet indices is coming through, might help to add descriptions to the figure that explicitly denotes this mapping. It is also unclear why this mapping is essential, and why it matters - those details are here below a bit, but might help to reorganize.}

\subsubsection{Bitrate Controller}
\label{sec:bitrate control}
So far, \namereparo has achieved compression by converting continuous features into discrete tokens that can be efficiently compressed by simply transmitting token indices. This process is relatively lossless except for errors in the decoder (\Sec{discrete decoder}). However, to further control the achieved bitrate as well as to teach \namereparo to not rely on all its tokens \ma{I'm not sure we want to mention the send point (teaching \namereparo to handle drops) at this point. The self-dropping used to teach the model is done during training, whereas the dropping for bitrate control is a test-time function. It's easier to just talk about bitrate control here, and discuss how we train the model later}, \namereparo performs ``self-dropping'', a mechanism to pseudo-randomly drop a fixed fraction of tokens across all packets of a frame to match the target bitrate. For example, if the target bitrate is \SI{200}{Kbps} and the bitrate of transmitting all tokens is \SI{300}{Kbps}, the bitrate controller will pseudo-randomly sample 1/3 tokens in each packet to drop. This ensures that \namereparo~can both adjust its bitrate as desired, and also learn that some tokens are inherently redundant and can be filled in if lost during training \ma{Again, I would not discuss training here; leave that for later}. In other words, it simultaneously achieves low-bitrate and loss-resilience.

However, if we simply randomly drop tokens in each packet, the receiver will be confused about the position of each received token in the $h\times w$ token map. Therefore, the tokens that get ``self-dropped'' in each packet are \ma{chosen deterministically based on the frame index and the packet index} pseudo-randomly sampled in that the sampling in each packet is determined by the frame index and packet index (\Fig{packetization} top row right). In practice, we implement this by setting the random seed for pseudo-random sampling in a packet to $n\times\text{frame index}+\text{packet index}$. As a result, the receiver only needs the frame index and packet index which are included in the header to know which tokens are dropped in each packet. With this information, the receiver can decode the locations of the tokens removed by the self-drop procedure (\Fig{packetization} bottom row left). %\vls{to the decoder, it doesn't matter whether the packet was self-dropped or dropped by the network right?, so why is the psuedo random sampling useful if the receiver doesn't need this info?} \tianhong{if the token is dropped by the network, we know where it is in the token map the network drops an entire packet. But if the token is self-dropped, the receiver needs to know where it is in the token map.} 
It then depacketizes each packet by reversing the deterministic mapping from \Sec{packetization} to form a $h\times w$ token map with missing tokens (\Fig{packetization} bottom row right), which are then filled in by the loss recovery module (\Sec{loss recovery}). Once the locations of missing tokens are identified, the receiver does not need to distinguish between those that were ``self-dropped'' \vs those that the network lost due to congestion; both are meant to be reconstructed by the loss recovery module in the same manner.

%\vls{This paragraph covers both how \namereparo itself does self-dropping in an effort to both make it more resilient, and how it achieves a certain bitrate. The way the text is written right now, the first part is not coming across. It is only really describing how the encoder transforms it into packets, and how the decoder realizes/maps which of the packets have been randomly dropped, but calling it reconstructed tokens makes me expect token generation which isn't done here if I'm correct. So it might help to split it into ``packetization'' and ``adaptive loss'' or something like that. It would also help if Figure 1 was made completely end-to-end with numbered modules that you could refer to here to make it clearer. You can then just discuss it briefly in an overview, and then talk about specific subsections.}


\subsubsection{Loss Recovery Module}
\label{sec:loss recovery}
\begin{figure}[t]
\begin{center}

\includegraphics[width=1.0\linewidth]{figures/mage}

\end{center}
\caption{Spatio-temporal loss recovery module. It uses a spatio-temporal vision transformer to recover any tokens that are lost using the received tokens in the last several frames.}\label{fig:mage}
\end{figure}

\noindent\textbf{Network Architecture.}  To reconstruct missing tokens from the received image tokens, the token map with missing tokens is fed into a Vision Transformer (ViT) \cite{vit} structure (\Fig{mage}). Transformers have become popular in computer vision and natural language processing tasks to predict missing image patches or words \cite{bert,vit,MAE} \ma{broken reference}. Vision Transformer, in particular, utilizes an attention module in each layer to aggregate information from all tokens in an image. \ma{Need to give more intuition here. Here is an attempt: To predict a missing token, the attention module uses the other received tokens, weighing them by their relevance to the missing token. It computes the relevance by performs a softmax over the dot product of each token with every other token (during training). We extend... I'm not sure if this is accurate, plz double check} The attention module simply performs a softmax over the dot product of each token with every other token to compute correspondences. We extend the standard vision transformer structure to video clips by using a spatio-temporal attention module \cite{arnab2021vivit}: in each transformer block, we first perform attention over the time dimension (across adjacent frames) and then perform attention over space dimension. This enables our loss reconstruction module to exploit both the spatial and temporal redundancy in the encoded video. Specifically, to reconstruct a missing token, it can use the nearby tokens both in space and across frames, as those tokens have a strong correlation with the missing token. Performing attention over time and space sequentially significantly reduces the computational cost: the attention over both space and time simultaneously requires $O(T^2h^2w^2)$ GPU memory, while attention first over time and then over space requires only $O(Th^2w^2 + T^2hw)$ GPU memory.
%\vls{is this new? do most people only do it simultaneously?} \tianhong{No, it is one common way to adapt transformer to videos.} 
%This significantly reduces the computational costs: the attention over both space and time simultaneously requires $O(T^2h^2w^2)$ GPU memory, while attention first over time and then over space requires only $O(Th^2w^2 + T^2hw)$ GPU memory.

%Our loss reconstruction module based on spatio-temporal ViT allows us to exploit both the spatial and temporal redundancy in the encoded video. To reconstruct a missing token, it can use the nearby tokens both in space and across frames, as those tokens have a strong correlation with the missing token. 

Leveraging temporal dependencies adds some overhead because the last few frames have to be held in memory to decode the next frame. Hence, we keep the temporal dependency to a minimum (\eg 6 frames). We note that using tokens from previous frames for loss recovery does not cause \namereparo to stall like traditional codecs due to undecodable frames. Specifically, the spatio-temporal ViT uses the 6 previous frames while decoding the current frame. This allows reuse of the received tokens across frames to achieve better bitrate and loss rate. However, every frame is still decoded irrespective of previous frame's reconstruction result merely based on the actually \emph{received tokens} of previous frames. If more tokens are lost in the previous frames, the quality of the current frame's reconstruction will be poorer, but \namereparo will never stop rendering or decoding unlike classical codecs. 
%\vls{we make a whole deal about standard codecs relying too much on temporal dependency earlier, how do we avoid that trap?}. \tianhong{The problem of previous codec is that, a subsequent frame cannot be rendered if one frame is lost. We avoid this kind of temporal dependency by using a per-frame codec. We harness temporal dependency to achieve lower bitrates / better loss recovery.} 
We include details of our spatio-temporal ViT structure in \Sec{loss-recovery-implementation}.


\noindent\textbf{Masking Strategy.} The goal with which we design \namereparo is to be resilient to losses across a range of bitrates. To enable adaptation to bitrates, we ``self-drop'' packets, in addition to any packet drops due to a congested network. During training time, the reconstruction module is taught to recover from both of these and fill in the lost tokens across dropped packets by simulating such drops. We simulate such drops by first simulating the packetization process and then, randomly sampling the self-drop ratio $r_d$ from 0 to 0.6 for every iteration. Based on this, we drop a certain fraction of tokens from each packet. Then, we randomly select a packet drop rate $r_p$ from 0 to 0.8, and randomly drop packets (and all tokens belonging to each dropped packet) based on the selected packet drop rate. The receiver first identifies which tokens (locations in the $h\times w$ grid) have been received based on frame and packet indices. The remaining missing tokens, either dropped due to ``self-drops'' or packet loss from congestion, are then filled in with a learnable mask token \texttt{[M]} (\Fig{model}) \vls{was this meant to have a figure} to denote tokens not received. This ensures that the input sequence length to the model is fixed regardless of the number of tokens dropped, a requirement for ViT. The filled token map is then combined with a positional embedding which provides the spatial location information for every token (including mask tokens) as the input of the ViT module. The output of the ViT module is a full $h\times w$ grid with reconstructed or original tokens in all its locations. Such tokens can be mapped back to features for the decoder after. 


\subsubsection{Discrete Decoder}
\label{sec:discrete decoder}
Finally, the reconstructed tokens are put back through a discrete decoder, which is the counterpart of the discrete encoder (\Sec{discrete encoder}). Each index in the reconstructed token is mapped back to its associated features from the codebook $Z$. This produces a set of  reconstructed discrete image features $\tilde{z}$ which may differ from the original quantized features $\hat{z}$ based on the extent of loss and ``self-drop''. The discrete features $\tilde{z}$ are treated like continuous features on the receiver, and put through a convolutional neural network (CNN) decoder $G$.
The decoder produces raw RGB images from the low-dimensional features $\tilde{z} \in \mathbb{R}^{C\times h \times w}$. The CNN decoder, like the encoder, uses several residual blocks\cite{resnet} and upsampling layers to produce the final image.

%\vls{this whole section seems to assume prior background on codebooks that makes it really hard to follow if you're not someone familiar with discrete encoders. I'd make this a little more clear using a first background, a description on losses, and a description of how it fits intol the video conferencing ecosystem.}

\subsection{\namereparo Model Details}
\subsubsection{Losses}
\label{sec:losses}
To train \namereparo, we incorporate a number of losses. For the neural codec, we use a vector-quantize loss between $z$ and $z_q$ that nudges the discrete features towards its continuous counterpart, a reconstruction loss (L1) between the input and final reconstructed frame, a perceptual loss~\cite{lpips} between input and reconstructed frame, and a discriminative loss between input and reconstructed frame. To aid with loss recovery, we use a reconstructive training loss which is a cross-entropy loss to recover the missing tokens. We briefly describe each of these below, but include more details in \Sec{implementation}.

\noindent\textbf{Vector-quantize Loss.} The vector-quantize loss is used to learn a codebook that better represents the encoded features. It achieves this by forcing the continuous features encoded by the encoder to be close to the nearest discrete features in the codebook. Formally, 

\begin{equation}
    \mathcal{L}_{VQ}(x, x_{rec}) = ||\textbf{sg}(z) - z_q || + \beta ||z - \textbf{sg}(z_q)||,
\end{equation}

where $\textbf{sg}$ represents stop-gradient operation. The second term is often denoted as "commitment loss" \cite{esser2021taming} and is designed in such a way that by fine-tuning $\beta$, we can control the "commitment level" between $z$ and $z_q$, \ie how fast $z$ moves toward $z_q$, and how fast $z_q$ moves toward $z$. \red{Once such a codebook is learned, it is fixed and shared between the transmitter and receiver in advance together with the other modules, so that we do not need to transmit them during video conferencing.}

\noindent\textbf{Perceptual Reconstruction Loss.} The major loss that forces our neural codec to reconstruct the original video frame is its reconstruction loss. We use a standard $L_1$ loss for reconstruction, i.e., 

\begin{equation}
    \mathcal{L}_{recon}(x, x_{rec}) = ||x - x_{rec}||_1.
\end{equation}

We also use a perceptual loss or LPIPS~\cite{lpips}, to force the reconstructed frame to be also perceptually similar to the original frame is the perceptual loss. It uses a pre-trained VGG network on ImageNet \cite{deng2009imagenet} as a feature extractor and extracts features from the original image and reconstructed image. It then computes the distance between the two features as the perceptual loss. This is meant to reflect how natural the image looks to the human eye. Consequently, our combined perceptual reconstruction loss is defined as 
\begin{equation}
    \mathcal{L}_{recon}(x, x_{rec}) = ||x - x_{rec}||_1 + \text{LPIPS}(x, x_{rec}).
\end{equation}

\noindent\textbf{Discriminative Loss.} We further use a patch-based discriminator \cite{isola2017image} $D$ that aims to differentiate between real and reconstructed images. Maximizing the discriminator loss minimizes the difference between $x$ and $x_{rec}$. The discriminative loss is defined as 

\begin{equation}
    \mathcal{L}_{D}(x, x_{rec}) = \log D(x) + \log(1 - D(x_{rec}))
\end{equation}

We then add all the above losses together for our complete training objective $Q^* = \{E^*, Z^*, G^* \}$ as:

\begin{equation}
\begin{split}
    Q^* = \argmin\limits_{E, Z, G} \max\limits_{D} \mathbb{E}_{x\sim p(x)}(\mathcal{L}_{VQ}(x, x_{rec}) & + \mathcal{L}_{recon}(x, x_{rec}) \\
    & + \mathcal{L}_{D}(x, x_{rec})).
\end{split}
\end{equation}

\noindent\textbf{Reconstructive Training Loss.} Let $\hat{z}=[\hat{z}_{ij}]_{i=1, j=1}^{h, w}$ denote the latent tokens obtained from the discrete encoder, and $M=[m_{ij}]_{i=1, j=1}^{h, w}$ denotes a corresponding binary mask denoting which tokens are received. The training objective is to reconstruct the masked tokens from the unmasked tokens. Therefore, we add a cross-entropy loss between the ground-truth one-hot tokens and the output of the decoder. Specifically,

\vspace{-5pt}
\begin{equation}
    \mathcal{L}_{reconstructive} = -\mathbb{E}_{\hat{z}} \big(\sum_{\forall i,j, m_{ij}=1} \log p(\hat{z}_{ij}|\hat{z}_{M})\big),
\end{equation}
where $\hat{z}_M$ are the (subset of) \emph{received} tokens in $\hat{z}$ and $p(\hat{z}_{ij}|\hat{z}_{M})$ is the probability distribution over the codebook for position $(i, j)$ in the token map predicted by the reconstruction network, conditioned on the input received tokens $\hat{z}_M$. Following common practice, we only optimize this loss on \emph{lost} tokens (optimizing the loss on all tokens reduces reconstruction performance, similar to the prior observations~\cite{MAE}).

\subsubsection{Inference Routine} As  the deadline for displaying each frame is hit every 33 ms for 30 fps, we aggregate all received packets for the current frame (as identified by the frame and packet indices) and regard all unreceived packets as lost. Once we place the tokens from all the received packets in their right places in the $h \times w$ token map, we know the exact locations of the missing tokens. We use all the tokens \emph{received} from the last 6 frames in their respective token maps to perform the spatio-temporal loss reconstruction (\Sec{loss recovery}). Given $p(z_q^i|z_q^{M})$ which is the probability distribution over the codebook predicted by the reconstruction network for position $(i, j)$ in the token map of the current frame given the received tokens, we choose the token with the highest probability as the reconstructed token for position $(i, j)$. The reconstructed token map is mapped to discrete features which are then fed into the neural decoder to generate the RGB frame to display.


%\subsection{Token-based Neural Codec}


%\subsubsection{Training and Inference} 

% \noindent\textbf{More training details.} Since the quantization step is nondifferentiable, to train the CNN encoder, we use straight-through gradient approximation which directly copies the gradient of $z_q$ to $z$. We use Adam optimizer \cite{xxx} to optimize our training loss. The detailed training recipe is included in the appendix \vls{point to appendix instead which is unlimited}.


%\subsection{Self-adaptive Packetization}
%\label{sec:packetization}


%\subsection{Spatiotemporal Loss Reconstruction}




==> source/related-0.tex <==
\section{Related Work}
\label{sec:related}

%\subsection{Video Codec for Videoconferencing}
%\noindent\textbf{Traditional Codec.}

%\noindent\textbf{Neural-based Video Codec.} 
\NewPara{Video Codecs.}
Most video applications use one of many classical codecs~\cite{vp8,vp9,h264,h265,av1} that use block-based motion prediction to compress video frames. Specifically, these codecs separate frames into keyframes (I-frames) that are compressed independently without any temporal correlations, and predicted frames (P-/B- frames) that are compressed based on deltas or differences relative to adjacent frames. These codecs are widely supported, and compress video very efficiently, especially in their slow modes. However, in their real-time modes for video conferencing, the achieved bitrate often exhibits a lot of variance around the target provided and does not compress too well. When classical codecs exceed the available capacity, they invariably cause packet loss and frame corruption~\cite{salsify}. To overcome some of these limitations, a number of neural codecs have been proposed in recent years~\cite{nas,srvc,swift,livenas,maxine,dvc}. Swift~\cite{swift} uses many levels, each encoded at a different bitrate, with learnt residuals at each level. NAS~\cite{nas}, LiveNAS~\cite{livenas} and SRVC~\cite{srvc} all use an underlying low-quality video that is enhanced using a Deep Neural Network (DNN) that may be static~\cite{nas}, updated periodically~\cite{srvc}, or fine-tuned online~\cite{livenas}.
However, most existing video codecs exploit temporal dependencies. As a result, one un-decodable or unrecoverable frame causes one or more subsequent frames to freeze. \namereparo eliminates the need for temporal dependency in its encoder and decoder, and only leverages it, when available, to improve the reconstruction quality. Therefore, even if one or two frames is un-decodable, it will not affect the subsequent frames, which practically removes video freezes.
% Recent years also have witnessed the prosperity of neural-based video codec. The pioneering DVC \cite{xxx} follows traditional codec. It uses optical flow network to generate prediction frame, then its residual with the current frame is coded. Many subsequent works also adopt this residual coding-based framework and refine the modules therein. For example, \cite{xxx, xxx, xx} proposed motion prediction to further reduce redundancy.

% Residual coding explicitly generates predicted frame in pixel domain as the context and only uses the subtraction to remove redundancy. By comparison, conditional coding has stronger extensibility. The definition, learning, and usage manner of condition can be flexibly designed. In \cite{xxx, xxx}, temporally conditional entropy models were designed. \cite{xxx} uses conditional coding to encode the foreground contents. \cite{xxx} proposed DCVC to learn feature domain contexts to increase context capacity. Then DCVC-TCM \cite{xxx} adopts feature propagation to boost performance. Recently, DCVC-HEM \cite{xxx} designs the hybrid entropy model utilizing both spatial and temporal contexts.



%\subsection{Loss Recovery for Video conferencing}

\noindent\textbf{FEC for Loss Recovery.} 
% From the early days of VoIP and Internet-based audio and video conferencing, FEC has played a key role in recovering lost packets \cite{xxx}. As standards for real-time media and conferencing developed, RTP payload formats for various FEC schemes were defined \cite{xxx}. Later, the FECFRAME working group of the IETF \cite{xxx} documented traditional FEC schemes such as parity codes \cite{xxx} and RS codes \cite{xxx}, as well as LDPC \cite{xxx} and Raptor codes \cite{xxx}. As the WebRTC project developed based on these standards, it also incorporated the use of FEC to protect media streams \cite{xxx}. All these codes are block codes. RS codes have the best loss recovery capabilities of any of them, including fountain \cite{xxx} and raptor codes \cite{xxx}. Recently, researchers also proposes to use streaming codes for FEC \cite{xxx}, achieving better loss recovery capability than block codes.
FEC, or Forward Error Correction, is a technique used in communication systems to recover lost data packets without the need for retransmission. Instead of requesting retransmission of lost packets, the receiver can use redundant information sent by the sender to reconstruct the original data. FEC is particularly important in real-time communication systems such as VoIP and video conferencing, where retransmission of lost packets can introduce unacceptable delays. Traditional FEC codes such as parity codes \cite{begen2010rtp}, Reed-Solomon (RS) codes \cite{reed1960polynomial}, and fountain codes \cite{mackay2005fountain} are all block codes. Many of these codes are optimal for random losses in which packets are lost independently. Recently, researchers have also proposed to use streaming codes for FEC and achieved better loss recovery capabilities than block codes for bursty losses, where several packets over one or more consecutive frames are lost.

To the best of our knowledge, we are the first to propose a neural-based loss recovery scheme for video conferencing. Instead of using FEC schemes which often introduce large bandwidth overheads, our scheme utilizes the inherent spatial and temporal redundancy of videos by first quantizing the videos into discrete tokens, and then reconstructing the lost tokens using whatever tokens that are received. Thus, we do not need to transmit redundant data packets for reconstruction.

\NewPara{Reconstructive Neural Networks.}
Recently, vision researchers have found that reconstructive learning, modeled after techniques in natural language processing e.g. \cite{devlin2018bert}, is a very effective task for learning visual representations in a self-supervised way. It uses a masked auto-encoder that reconstructs masked images as a pre-training task \cite{bao2021beit, MAE}. However, such reconstructive-based self-supervised learning methods typically focus more on the quality of the learned intermediate representations instead of the reconstructed images. As a result, they care more about learning the overall semantics of the image instead of reconstructing the details, which often leads to blurry and low-quality reconstructions \cite{MAE}.

Another line of work using reconstructive neural networks is in image synthesis. It first encodes the image into a low-dimensional feature space using a neural encoder. It then uses a feature codebook to quantize the encoded features into token maps. Such token maps are typically highly compressed compared to the original images. It finally uses a neural decoder to reconstruct the original image using such token maps \cite{razavi2019generating, yu2021vector, chang2022maskgit, esser2021taming}. Researchers further use multiple techniques such as perceptual \cite{esser2021taming} loss and discriminative training \cite{yu2021vector} to force the token maps to reconstruct clear and detailed images. Motivated by this, \cite{li2022mage} performs reconstructive self-supervised learning on the token level instead of the pixel level. It masks the input token maps instead of the raw images and uses a cross-entropy loss to force the reconstructive network to predict masked tokens. Such design helps it achieves high-quality image reconstructions even under a high masking ratio (e.g., 75\%).

These works show the inherent spatial redundancy of images: one image can be represented and reconstructed by only a few discrete tokens, and missing pixels of an image can be largely recovered by its surrounding context. This property perfectly fits a loss-resilient video codec: a video can be represented by a few discrete tokens, and any loss of these tokens can be recovered by the surrounding tokens. Thus, we propose \namereparo, the first neural-based loss-resilient codec for video conferencing.
